Screening in gated bilayer graphene via variational calculus

We analyze the response of bilayer graphene to an external transverse electric field using a variational method. A previous attempt to do so in a recent paper by Falkovsky [Phys. Rev. B 80, 113413 (2009)] is shown to be flawed. Our calculation reaffirms the original results obtained by one of us [E. McCann, Phys. Rev. B 74, 161403(R) (2006)] by a different method. Finally, we generalize these original results to describe a dual-gated bilayer graphene device.

==> Falkovsky_bbl.tex <==
%Merlin.mbs v4.21 2009-07-09.
\begin{thebibliography}{10}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \ifx #1\undefined \expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
\fi
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
\fi
}%
\providecommand \enquote [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand\href[0]{\@sanitize\@href}%
\providecommand\@href[1]{\endgroup\@@startlink{#1}\endgroup\@@href}%
\providecommand\@@href[1]{#1\@@endlink}%
\providecommand \@sanitize [0]{\begingroup\catcode`\&12\catcode`\#12\relax}%
\@ifxundefined \pdfoutput {\@firstoftwo}{%
 \@ifnum{\z@=\pdfoutput}{\@firstoftwo}{\@secondoftwo}%
}{%
 \providecommand\@@startlink[1]{\leavevmode\special{html:<a href="#1">}}%
 \providecommand\@@endlink[0]{\special{html:</a>}}%
}{%
 \providecommand\@@startlink[1]{%
  \leavevmode
  \pdfstartlink
   attr{/Border[0 0 1 ]/H/I/C[0 1 1]}%
   user{/Subtype/Link/A<</Type/Action/S/URI/URI(#1)>>}%
  \relax
 }%
 \providecommand\@@endlink[0]{\pdfendlink}%
}%
\providecommand \url  [0]{\begingroup\@sanitize \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix}}%
\providecommand \urlprefix [0]{URL }%
\providecommand \Eprint[0]{\href }%
\@ifxundefined \urlstyle {%
  \providecommand \doi [1]{doi:\discretionary{}{}{}#1}%
}{%
  \providecommand \doi [0]{doi:\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url }%
}%
\providecommand \doibase [0]{http://dx.doi.org/}%
\providecommand \Doi[1]{\href{\doibase#1}}%
\providecommand \bibAnnote [3]{%
  \BibitemShut{#1}%
  \begin{quotation}\noindent
    \textsc{Key:}\ #2\\\textsc{Annotation:}\ #3%
  \end{quotation}%
}%
\providecommand \bibAnnoteFile [2]{%
  \IfFileExists{#2}{\bibAnnote {#1} {#2} {\input{#2}}}{}%
}%
\providecommand \typeout [0]{\immediate \write \m@ne }%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo [0]{\@secondoftwo}%
\providecommand \bibfield [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen[0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut [1]{\csname bibitem#1\endcsname}%
%</preamble>
\bibitem{Castroneto2009tep}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{A.~H.}\ \bibnamefont{Castro~Neto}}, \bibinfo
  {author} {\bibfnamefont{F.}~\bibnamefont{Guinea}}, \bibinfo {author}
  {\bibfnamefont{N.~M.~R.}\ \bibnamefont{Peres}}, \bibinfo {author}
  {\bibfnamefont{K.~S.}\ \bibnamefont{Novoselov}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~K.}\ \bibnamefont{Geim}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/RevModPhys.81.109}{\bibinfo {journal} {Rev. Mod. Phys.}}\ }%
  \textbf{\bibinfo {volume} {81}},\ \bibinfo {pages} {109} (\bibinfo {year}
  {2009})%
  \bibAnnoteFile{NoStop}{Castroneto2009tep}%
\bibitem{McCann2006lld}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{E.}~\bibnamefont{McCann}}\ and\ \bibinfo
  {author} {\bibfnamefont{V.~I.}\ \bibnamefont{Fal'ko}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevLett.96.086805}{\bibinfo {journal} {Phys. Rev. Lett.}}\
  }%
  \textbf{\bibinfo {volume} {96}},\ \bibinfo {eid} {086805} (\bibinfo {year}
  {2006})%
  \bibAnnoteFile{NoStop}{McCann2006lld}%
\bibitem{Castro2007bbg}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{E.~V.}\ \bibnamefont{Castro}}, \bibinfo
  {author} {\bibfnamefont{K.~S.}\ \bibnamefont{Novoselov}}, \bibinfo {author}
  {\bibfnamefont{S.~V.}\ \bibnamefont{Morozov}}, \bibinfo {author}
  {\bibfnamefont{N.~M.~R.}\ \bibnamefont{Peres}}, \bibinfo {author}
  {\bibfnamefont{J.~M. B.~L.}\ \bibnamefont{dos Santos}}, \bibinfo {author}
  {\bibfnamefont{J.}~\bibnamefont{Nilsson}}, \bibinfo {author}
  {\bibfnamefont{F.}~\bibnamefont{Guinea}}, \bibinfo {author}
  {\bibfnamefont{A.~K.}\ \bibnamefont{Geim}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~H.}\ \bibnamefont{Castro~Neto}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevLett.99.216802}{\bibinfo {journal} {Phys. Rev. Lett.}}\
  }%
  \textbf{\bibinfo {volume} {99}},\ \bibinfo {eid} {216802} (\bibinfo {year}
  {2007})%
  \bibAnnoteFile{NoStop}{Castro2007bbg}%
\bibitem{McCann2006agi}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{E.}~\bibnamefont{McCann}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.74.161403}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {74}},\ \bibinfo {eid} {161403} (\bibinfo {year}
  {2006})%
  \bibAnnoteFile{NoStop}{McCann2006agi}%
\bibitem{Ohta2006ces}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{T.}~\bibnamefont{Ohta}}, \bibinfo {author}
  {\bibfnamefont{A.}~\bibnamefont{Bostwick}}, \bibinfo {author}
  {\bibfnamefont{T.}~\bibnamefont{Seyller}}, \bibinfo {author}
  {\bibfnamefont{K.}~\bibnamefont{Horn}},\ and\ \bibinfo {author}
  {\bibfnamefont{E.}~\bibnamefont{Rotenberg}},\ }%
  \bibfield{journal}{%
  \Doi{10.1126/science.1130681}{\bibinfo {journal} {Science}}\ }%
  \textbf{\bibinfo {volume} {313}},\ \bibinfo {pages} {951} (\bibinfo {year}
  {2006})%
  \bibAnnoteFile{NoStop}{Ohta2006ces}%
\bibitem{Oostinga2007gii}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{J.~B.}\ \bibnamefont{Oostinga}}, \bibinfo
  {author} {\bibfnamefont{H.~B.}\ \bibnamefont{Heersche}}, \bibinfo {author}
  {\bibfnamefont{X.}~\bibnamefont{Liu}}, \bibinfo {author}
  {\bibfnamefont{A.~F.}\ \bibnamefont{Morpurgo}},\ and\ \bibinfo {author}
  {\bibfnamefont{L.~M.~K.}\ \bibnamefont{Vandersypen}},\ }%
  \bibfield{journal}{%
  \Doi{doi:10.1038/nmat2082}{\bibinfo {journal} {Nature Mat.}}\ }%
  \textbf{\bibinfo {volume} {7}},\ \bibinfo {pages} {151} (\bibinfo {year}
  {2008})%
  \bibAnnoteFile{NoStop}{Oostinga2007gii}%
\bibitem{Henriksen2008cri}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{E.~A.}\ \bibnamefont{Henriksen}}, \bibinfo
  {author} {\bibfnamefont{Z.}~\bibnamefont{Jiang}}, \bibinfo {author}
  {\bibfnamefont{L.-C.}\ \bibnamefont{Tung}}, \bibinfo {author}
  {\bibfnamefont{M.~E.}\ \bibnamefont{Schwartz}}, \bibinfo {author}
  {\bibfnamefont{M.}~\bibnamefont{Takita}}, \bibinfo {author}
  {\bibfnamefont{Y.-J.}\ \bibnamefont{Wang}}, \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Kim}},\ and\ \bibinfo {author}
  {\bibfnamefont{H.~L.}\ \bibnamefont{Stormer}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevLett.100.087403}{\bibinfo {journal} {Phys. Rev. Lett.}}\
  }%
  \textbf{\bibinfo {volume} {100}},\ \bibinfo {eid} {087403} (\bibinfo {year}
  {2008})%
  \bibAnnoteFile{NoStop}{Henriksen2008cri}%
\bibitem{Li2008dcd}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{Z.~Q.}\ \bibnamefont{Li}}, \bibinfo {author}
  {\bibfnamefont{E.~A.}\ \bibnamefont{Henriksen}}, \bibinfo {author}
  {\bibfnamefont{Z.}~\bibnamefont{Jiang}}, \bibinfo {author}
  {\bibfnamefont{Z.}~\bibnamefont{Hao}}, \bibinfo {author}
  {\bibfnamefont{M.~C.}\ \bibnamefont{Martin}}, \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Kim}}, \bibinfo {author}
  {\bibfnamefont{H.~L.}\ \bibnamefont{Stormer}},\ and\ \bibinfo {author}
  {\bibfnamefont{D.~N.}\ \bibnamefont{Basov}},\ }%
  \bibfield{journal}{%
  \Doi{10.1038/nphys989}{\bibinfo {journal} {Nat. Phy.}}\ }%
  \textbf{\bibinfo {volume} {4}},\ \bibinfo {pages} {532} (\bibinfo {year}
  {2008})%
  \bibAnnoteFile{NoStop}{Li2008dcd}%
\bibitem{Zhang2009doo}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{Y.}~\bibnamefont{Zhang}}, \bibinfo {author}
  {\bibfnamefont{T.-T.}\ \bibnamefont{Tang}}, \bibinfo {author}
  {\bibfnamefont{C.}~\bibnamefont{Girit}}, \bibinfo {author}
  {\bibfnamefont{Z.}~\bibnamefont{Hao}}, \bibinfo {author}
  {\bibfnamefont{M.~C.}\ \bibnamefont{Martin}}, \bibinfo {author}
  {\bibfnamefont{A.}~\bibnamefont{Zettl}}, \bibinfo {author}
  {\bibfnamefont{M.~F.}\ \bibnamefont{Crommie}}, \bibinfo {author}
  {\bibfnamefont{Y.~R.}\ \bibnamefont{Shen}},\ and\ \bibinfo {author}
  {\bibfnamefont{F.}~\bibnamefont{Wang}},\ }%
  \bibfield{journal}{%
  \Doi{10.1038/nature08105}{\bibinfo {journal} {Nature}}\ }%
  \textbf{\bibinfo {volume} {459}},\ \bibinfo {pages} {820} (\bibinfo {year}
  {2009})%
  \bibAnnoteFile{NoStop}{Zhang2009doo}%
\bibitem{Mak2009ooa}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{K.~F.}\ \bibnamefont{Mak}}, \bibinfo
  {author} {\bibfnamefont{C.~H.}\ \bibnamefont{Lui}}, \bibinfo {author}
  {\bibfnamefont{J.}~\bibnamefont{Shan}},\ and\ \bibinfo {author}
  {\bibfnamefont{T.~F.}\ \bibnamefont{Heinz}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevLett.102.256405}{\bibinfo {journal} {Phys. Rev. Lett.}}\
  }%
  \textbf{\bibinfo {volume} {102}},\ \bibinfo {eid} {256405} (\bibinfo {year}
  {2009})%
  \bibAnnoteFile{NoStop}{Mak2009ooa}%
\bibitem{Kuzmenko2009iso}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{A.~B.}\ \bibnamefont{Kuzmenko}}, \bibinfo
  {author} {\bibfnamefont{E.}~\bibnamefont{van Heumen}}, \bibinfo {author}
  {\bibfnamefont{D.}~\bibnamefont{van~der Marel}}, \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Lerch}}, \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Blake}}, \bibinfo {author}
  {\bibfnamefont{K.~S.}\ \bibnamefont{Novoselov}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~K.}\ \bibnamefont{Geim}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.79.115441}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {79}},\ \bibinfo {eid} {115441} (\bibinfo {year}
  {2009})%
  \bibAnnoteFile{NoStop}{Kuzmenko2009iso}%
\bibitem{Kuzmenko2009dot}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{A.~B.}\ \bibnamefont{Kuzmenko}}, \bibinfo
  {author} {\bibfnamefont{I.}~\bibnamefont{Crassee}}, \bibinfo {author}
  {\bibfnamefont{D.}~\bibnamefont{van~der Marel}}, \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Blake}},\ and\ \bibinfo {author}
  {\bibfnamefont{K.~S.}\ \bibnamefont{Novoselov}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.80.165406}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {80}},\ \bibinfo {eid} {165406} (\bibinfo {year}
  {2009})%
  \bibAnnoteFile{NoStop}{Kuzmenko2009dot}%
\bibitem{Kuzmenko2009gti}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{A.~B.}\ \bibnamefont{Kuzmenko}}, \bibinfo
  {author} {\bibfnamefont{L.}~\bibnamefont{Benfatto}}, \bibinfo {author}
  {\bibfnamefont{E.}~\bibnamefont{Cappelluti}}, \bibinfo {author}
  {\bibfnamefont{I.}~\bibnamefont{Crassee}}, \bibinfo {author}
  {\bibfnamefont{D.}~\bibnamefont{van~der Marel}}, \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Blake}}, \bibinfo {author}
  {\bibfnamefont{K.~S.}\ \bibnamefont{Novoselov}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~K.}\ \bibnamefont{Geim}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevLett.103.116804}{\bibinfo {journal} {Phys. Rev. Lett.}}\
  }%
  \textbf{\bibinfo {volume} {103}},\ \bibinfo {eid} {116804} (\bibinfo {year}
  {2009})%
  \bibAnnoteFile{NoStop}{Kuzmenko2009gti}%
\bibitem{Zhao2010sbi}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{Y.}~\bibnamefont{Zhao}}, \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Cadden-Zimansky}}, \bibinfo {author}
  {\bibfnamefont{Z.}~\bibnamefont{Jiang}},\ and\ \bibinfo {author}
  {\bibfnamefont{P.}~\bibnamefont{Kim}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevLett.104.066801}{\bibinfo {journal} {Phys. Rev. Lett.}}\
  }%
  \textbf{\bibinfo {volume} {104}},\ \bibinfo {pages} {066801} (\bibinfo {year}
  {2010})%
  \bibAnnoteFile{NoStop}{Zhao2010sbi}%
\bibitem{Kim2009qhe}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{S.}~\bibnamefont{Kim}}\ and\ \bibinfo
  {author} {\bibfnamefont{E.}~\bibnamefont{Tutuc}},\ }%
  \enquote{\bibinfo {title} {Quantum hall effect in dual-gated graphene
  bilayers with tunable layer density imbalance},}\
  \Eprint{http://arxiv.org/abs/0909.2288}{arXiv:0909.2288}%
  \bibAnnoteFile{NoStop}{Kim2009qhe}%
\bibitem{Nilsson2006eei}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{J.}~\bibnamefont{Nilsson}}, \bibinfo
  {author} {\bibfnamefont{A.~H.}\ \bibnamefont{Castro~Neto}}, \bibinfo {author}
  {\bibfnamefont{N.~M.~R.}\ \bibnamefont{Peres}},\ and\ \bibinfo {author}
  {\bibfnamefont{F.}~\bibnamefont{Guinea}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.73.214418}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {73}},\ \bibinfo {pages} {214418} (\bibinfo {year}
  {2006})%
  \bibAnnoteFile{NoStop}{Nilsson2006eei}%
\bibitem{Min2007ait}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{H.}~\bibnamefont{Min}}, \bibinfo {author}
  {\bibfnamefont{B.}~\bibnamefont{Sahu}}, \bibinfo {author}
  {\bibfnamefont{S.~K.}\ \bibnamefont{Banerjee}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~H.}\ \bibnamefont{MacDonald}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.75.155115}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {75}},\ \bibinfo {pages} {155115} (\bibinfo {year}
  {2007})%
  \bibAnnoteFile{NoStop}{Min2007ait}%
\bibitem{McCann2007eib}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{E.}~\bibnamefont{McCann}}, \bibinfo {author}
  {\bibfnamefont{D.}~\bibnamefont{Abergel}},\ and\ \bibinfo {author}
  {\bibfnamefont{V.}~\bibnamefont{Fal'ko}},\ }%
  \bibfield{journal}{%
  \Doi{doi:10.1016/j.ssc.2007.03.054}{\bibinfo {journal} {Solid State
  Commun.}}\ }%
  \textbf{\bibinfo {volume} {143}},\ \bibinfo {pages} {110} (\bibinfo {year}
  {2007})%
  \bibAnnoteFile{NoStop}{McCann2007eib}%
\bibitem{Nilsson2008epo}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{J.}~\bibnamefont{Nilsson}}, \bibinfo
  {author} {\bibfnamefont{A.~H.}\ \bibnamefont{Castro~Neto}}, \bibinfo {author}
  {\bibfnamefont{F.}~\bibnamefont{Guinea}},\ and\ \bibinfo {author}
  {\bibfnamefont{N.~M.~R.}\ \bibnamefont{Peres}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.78.045405}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {78}},\ \bibinfo {pages} {045405} (\bibinfo {year}
  {2008})%
  \bibAnnoteFile{NoStop}{Nilsson2008epo}%
\bibitem{Zhang2008dot}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{L.~M.}\ \bibnamefont{Zhang}}, \bibinfo
  {author} {\bibfnamefont{Z.~Q.}\ \bibnamefont{Li}}, \bibinfo {author}
  {\bibfnamefont{D.~N.}\ \bibnamefont{Basov}}, \bibinfo {author}
  {\bibfnamefont{M.~M.}\ \bibnamefont{Fogler}}, \bibinfo {author}
  {\bibfnamefont{Z.}~\bibnamefont{Hao}},\ and\ \bibinfo {author}
  {\bibfnamefont{M.~C.}\ \bibnamefont{Martin}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.78.235408}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {78}},\ \bibinfo {eid} {235408} (\bibinfo {year}
  {2008})%
  \bibAnnoteFile{NoStop}{Zhang2008dot}%
\bibitem{Falkovsky2009sig}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{L.~A.}\ \bibnamefont{Falkovsky}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.80.113413}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {80}},\ \bibinfo {pages} {113413} (\bibinfo {year}
  {2009})%
  \bibAnnoteFile{NoStop}{Falkovsky2009sig}%
\bibitem{Bello1981dol}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{M.~S.}\ \bibnamefont{Bello}}, \bibinfo
  {author} {\bibfnamefont{E.~I.}\ \bibnamefont{Levin}}, \bibinfo {author}
  {\bibfnamefont{B.~I.}\ \bibnamefont{Shklovskii}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~L.}\ \bibnamefont{Efros}},\ }%
  \bibfield{journal}{%
  \bibinfo {journal} {Sov. Phys. JETP}\ }%
  \textbf{\bibinfo {volume} {53}},\ \bibinfo {pages} {822} (\bibinfo {year}
  {1981})%
  \bibAnnoteFile{NoStop}{Bello1981dol}%
\bibitem{Dolgov1981oaa}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{O.~V.}\ \bibnamefont{Dolgov}}, \bibinfo
  {author} {\bibfnamefont{D.~A.}\ \bibnamefont{Kirzhnits}},\ and\ \bibinfo
  {author} {\bibfnamefont{E.~G.}\ \bibnamefont{Maksimov}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/RevModPhys.53.81}{\bibinfo {journal} {Rev. Mod. Phys.}}\ }%
  \textbf{\bibinfo {volume} {53}},\ \bibinfo {pages} {81} (\bibinfo {year}
  {1981})%
  \bibAnnoteFile{NoStop}{Dolgov1981oaa}%
\bibitem{Eisenstein1994cot}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{J.~P.}\ \bibnamefont{Eisenstein}}, \bibinfo
  {author} {\bibfnamefont{L.~N.}\ \bibnamefont{Pfeiffer}},\ and\ \bibinfo
  {author} {\bibfnamefont{K.~W.}\ \bibnamefont{West}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.50.1760}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {50}},\ \bibinfo {pages} {1760} (\bibinfo {year}
  {1994})%
  \bibAnnoteFile{NoStop}{Eisenstein1994cot}%
\bibitem{Min2007pmi}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{H.}~\bibnamefont{Min}}, \bibinfo {author}
  {\bibfnamefont{G.}~\bibnamefont{Borghi}}, \bibinfo {author}
  {\bibfnamefont{M.}~\bibnamefont{Polini}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~H.}\ \bibnamefont{MacDonald}},\ }%
  \bibfield{journal}{%
  \Doi{10.1103/PhysRevB.77.041407}{\bibinfo {journal} {Phys. Rev. B}}\ }%
  \textbf{\bibinfo {volume} {77}},\ \bibinfo {pages} {041407(R)} (\bibinfo
  {year} {2008})%
  \bibAnnoteFile{NoStop}{Min2007pmi}%
\bibitem{Zhang2009eei}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{F.}~\bibnamefont{Zhang}}, \bibinfo {author}
  {\bibfnamefont{H.}~\bibnamefont{Min}}, \bibinfo {author}
  {\bibfnamefont{M.}~\bibnamefont{Polini}},\ and\ \bibinfo {author}
  {\bibfnamefont{A.~H.}\ \bibnamefont{MacDonald}},\ }%
  \enquote{\bibinfo {title} {Electron-electron interactions in graphene
  bilayers},}\ \bibinfo {note} {ArXiv:0907.2448 (unpublished)}%
  \bibAnnoteFile{NoStop}{Zhang2009eei}%
\bibitem{Nandkishore2009fte}%
  \BibitemOpen
  \bibfield{author}{%
  \bibinfo {author} {\bibfnamefont{R.}~\bibnamefont{Nandkishore}}\ and\
  \bibinfo {author} {\bibfnamefont{L.~S.}\ \bibnamefont{Levitov}},\ }%
  \enquote{\bibinfo {title} {Ferroelectric-type excitonic instability in
  bilayer graphene},}\
  \Eprint{http://arxiv.org/abs/0907.5395}{arXiv:0907.5395}%
  \bibAnnoteFile{NoStop}{Nandkishore2009fte}%
\end{thebibliography}%

